State-of-the-Art HCI for Dementia Care: A Scoping Review of Recent Technological Advances

Dementia significantly impacts cognitive, behavioral, and functional abilities, creating challenges for both individuals and caregivers. Recent advancements in HCI have introduced innovative technological solutions to support people with dementia (PwD) and their caregivers. This scoping review systematically examines 32 recent publications from leading digital libraries, categorizing technological interventions into four key domains: Assistive and Smart Technology for Daily Life, Social Interaction and Communication, Well-being and Psychological Support, and Caregiver Support and Training. Our analysis highlights how emerging technologies are transforming dementia care. These technologies enhance quality of life by promoting independence, fostering social engagement, and providing emotional and cognitive support. However, the review also identifies critical gaps, particularly in addressing the needs of individuals with early-stage dementia and the lack of individualized support mechanisms. By emphasizing user-centered design, accessibility, and ethical considerations, this paper offers a structured roadmap for future research and practice in dementia care. It bridges the gap between technological innovation and the real-world needs of PwD and their caregivers, providing valuable insights for researchers, practitioners, and policymakers. This review not only synthesizes current advancements but also sets the stage for future HCI-driven innovations in dementia care, aiming to improve outcomes for an aging global population.

==> Sections/Background.tex <==
\section{Background}
As aforementioned, dementia is a complicated syndrome characterized by a decline in cognitive function that presents a major worldwide healthcare concern. In recent years, the issue of dementia care has broadened, placing growing demands on individuals, families, and healthcare systems, particularly in the context of our aging population. This section begins with a succinct introduction of dementia care, followed by a presentation of existing research and the up-to-date technologies employed in the field of dementia care.


\subsection{Dementia Care}
\subsubsection{Dementia Types} 
In general, dementia types can be divided into six major categories: mold cognitive impairment (MCI), Alzheimer's disease (AD), Parkinson's disease dementia (PDD), Lewy body dementia (LBD), frontotemporal dementia (FTD), and Creutzfeldt-Jakob disease (CJD)~\cite{ono2023mortality,manzine2022potential,magdy2022cognitive,mehraram2020weighted,gublood}. MCI and Alzheimer's disease are the most prevalent dementia types. MCI is a stage of cognitive impairment that is visible but not severe enough to be categorized as dementia~\cite{portet2006mild}. It can be considered a transitional phase between normal aging and dementia. 
Alzheimer's is the most well-known form of dementia, characterized by progressive memory loss and cognitive decline ~\cite{cummings2002alzheimer}. Many studies in our literature review research referenced these two types of dementia. Moreover, these classifications provide vital insights into the diverse landscape of dementia, aiding in accurate diagnosis and tailored care.

\subsubsection{Dementia Diagnosis}
The process of diagnosing dementia entails assessing cognitive decline and the impact of this decline on an individual's daily activities~\cite{arvanitakis2019diagnosis}. This evaluation is typically conducted by a clinician and involves a thorough history assessment and a comprehensive mental status examination. 
To initiate the cognitive assessment, brief cognitive impairment screening questionnaires can be employed~\cite{weintraub2022neuropsychological}. Further diagnostic insight can be gleaned through the use of neuropsychological testing \cite{jacova2007neuropsychological}. In addition to these cognitive assessments, physical examinations and brain neuroimaging serve as invaluable diagnostic tools in identifying the etiology of dementia, including conditions, such as stroke or structural alterations within the brain ~\cite{arvanitakis2019diagnosis}. However, it's important to acknowledge that achieving a highly accurate clinical dementia diagnosis can be a formidable challenge, especially during the early stages when relying solely on these approaches. In response to this challenge, recent advancements in AI have brought forth promising developments.  
Merl et al.~\cite{merl2022truth} demonstrate how AI algorithms, coupled with conventional magnetic resonance imaging (MRI), hold potential for significantly enhancing diagnostic accuracy across various dementia types.
Furthermore, there is an emerging landscape of innovative methods and techniques that have the potential to be harnessed for multi-modal dementia diagnosis. Palliya et al.~\cite{palliya2021advances} presented the use of speech features, facial expressions, movement patterns, sleep behavior, and mood changes as promising avenues in this quest for improved diagnostic precision. 
Using clinical dementia diagnosis combined with existing artificial intelligence, wearable technology, and multi-modal behavior analysis, it is feasible to conduct an early-stage diagnosis of dementia with promising results. 

\subsubsection{Conventional Dementia Care} 
Dementia care represents a multifaceted challenge within the realm of dementia research. Traditional dementia care primarily focuses on two key objectives: enhancing overall well-being and promoting independence for as long as possible to delay the necessity of placing individuals in long-term care institutions ~\cite{rappe2005influence}. PwD receive day-to-day care from healthcare professionals who monitor their vital signs and address any behavioral or psychiatric issues that may arise. Additionally, regular medical check-ups are conducted by physicians to ensure comprehensive healthcare management.
Caregivers play an indispensable role in improving the quality of life of PwD throughout the course of the illness. They track the progression of the disease, assist with medication management, implement fall prevention strategies, engage patients in daily activities, and offer emotional support, with a focus on stress reduction~\cite{abdollahpour2018positive}. Formal caregiver interventions encompass a wide range of approaches, including psycho-education, support groups, individual counseling, and respite care programs~\cite{chien2005effectiveness}.
These interventions extend beyond healthcare considerations, emphasizing non-health-related benefits, such as enhanced understanding of the illness, improved communication, and a more positive dynamic between caregiver and patient. These efforts finally aim to enhance the overall quality of life for both the patient and the caregiver.


However, the intricate mechanisms underlying dementia remain a subject of ongoing research, and our understanding in this field is far from complete. 
PwD frequently undergo fluctuations in their symptoms~\cite{livingston2020dementia} and conventional diagnostic tools often struggle to capture these dynamic changes. This presents a significant challenge, as it can complicate the provision of effective dementia care.
Moreover, the demands of day-to-day healthcare for individuals with dementia can place considerable stress on caregivers, both emotionally and financially, making it a burdensome undertaking for many families. As a result, some early-stage people living with dementia may opt for in-home healthcare as an alternative. However, limited experience in dementia care can significantly compound the challenges faced by informal caregivers. 
Due to these challenges, a range of technologies, including assistive devices, telehealth and remote monitoring, robotics, sensory and environmental enhancements, among others, have emerged as promising solutions to provide valuable support for dementia care.

\subsection{The Advancements of Technologies in Dementia Care}
In general, PwD often receive appropriate care in clinical settings; however, providing the same level of care in a home environment poses unique challenges. Informal caregivers, who are frequently family members, even if the PwD lives alone, may have limited experience in dementia care. This presents a pressing need to enhance the well-being of PwD and provide comprehensive training for dementia caregivers.
To address these challenges, existing technologies have provided valuable alternatives, making substantial contributions to dementia care and enhancing the quality of life for both patients and caregivers. These advancements have taken shape in various dimensions, spanning diagnosis, treatment, monitoring, and support. Particularly, monitoring and support hold a pivotal role in the landscape of dementia care. 
As mentioned in a recent research by Wrede et al.~\cite{wrede2022create}, there is a rising investigation into Unobtrusive Monitoring (UM) technology to allow the extended independent life of PwD in their homes. These technologies are intended to remotely monitor the lifestyle, health, and safety of PwD, providing advantages such as objective surveillance and prompt interventions. However, they also raise considerations such as potential information overload and reduced human interaction~\cite{mclaughlin2022evaluating}.
Moreover, several support technologies, such as assistive technologies for PwD and their caregivers~\cite{ienca2018ethical,sriram2020carers}, can enhance their quality of life as well.


As Artificial Intelligence (AI), Large Language Models (LLMs), Wearable Technologies, Robotics, and other cutting-edge innovations continue to advance, they offer substantial potential for integration into existing dementia care technologies. These innovative solutions have the power to significantly enhance the well-being of PwD and their caregivers. Simultaneously, they can alleviate the burden on both families and healthcare institutions. The advantages of these technologies serve as a compelling motivation for us to conduct comprehensive literature review studies and embark on explorations into the future of research in dementia care. Their transformative impact on the field holds great promise for improving the lives of PwD and their caregivers while optimizing the overall care ecosystem.
